Skeletons and Minimum Energy Scheduling

Consider the problem where $n$ jobs, each with a release time, a deadline and a required processing time are to be feasibly scheduled in a single- or multi-processor setting so as to minimize the total energy consumption of the schedule. A processor has two available states: a \emph{sleep state} where no energy is consumed but also no processing can take place, and an \emph{active state} which consumes energy at a rate of one, and in which jobs can be processed. Transitioning from the active to the sleep does not incur any further energy cost, but transitioning from the sleep to the active state requires $q$ energy units. Jobs may be preempted and (in the multi-processor case) migrated. The single-processor case of the problem is known to be solvable in polynomial time via an involved dynamic program, whereas the only known approximation algorithm for the multi-processor case attains an approximation factor of $3$ and is based on rounding the solution to a linear programming relaxation of the problem. In this work, we present efficient and combinatorial approximation algorithms for both the single- and the multi-processor setting. Before, only an algorithm based on linear programming was known for the multi-processor case. Our algorithms build upon the concept of a \emph{skeleton}, a basic (and not necessarily feasible) schedule that captures the fact that some processor(s) must be active at some time point during an interval. Finally, we further demonstrate the power of skeletons by providing an $2$-approximation algorithm for the multiprocessor case, thus improving upon the recent breakthrough $3$-approximation result. Our algorithm is based on a novel rounding scheme of a linear-programming relaxation of the problem which incorporates skeletons.

==> approximation.tex <==


%\maketitle


\section{A 3/2 Approximation Algorithm}
Consider a fractional optimal solution. Let there be $b$ solutions: $\mathcal{C}^1,\dots,\mathcal{C}^b$. Wlog let $\mathcal{C}^1$ be the least cost solution. We now schedule jobs (integrally) to this solution as much as possible. Let $U$ denote the set of unfilled jobs, i.e., those jobs which are partially or completely not scheduled.  

We will now partition the set of jobs $U$ as well as the time interval $[0,D]$. Let $T$ be the set of time slots which is contained in some jobs of $U$. Suppose $T = \cup_{i = 1}^{r}T_i$  be such that each $T_i$ is contiguous and each  $T_i$ and $T_j$ are disjoint. Let $T_i = [p_i,q_i]$ such that $q_i < p_{i+1}$. Any job in $U$ will be contained in exactly one of $T_i$. Let $ U = \cup_{i =1}^{r} U_i$ be such that $U_i$ is set of all jobs contained in $T_i$. In our integral solution, all time slots in $T_i$ are filled (because each time slot in $T_i$ is contained in some job of $U_i$). The set $T$ partition the interval $[0,D]$ into many time segments: $[0,p_1], [p_1,q_1], \dots, [q_r,D]$. The time segments $[p_1,q_1],\dots,[p_r,q_r]$ are called good segments and the time segments $[0,p_1],[q_1,p_2],\dots,[q_r,D]$ are called bad segments. Let for any set of time slots $R$, $|\mathcal{C}^i(R)| = |\mathcal{C}^i \cap R|$ be the total length of intervals of solution $\mathcal{C}^i$ inside $R$ (and $\mathcal{C}^i(R)$ denotes the  portions of intervals of $\mathcal{C}^i$ inside $R$).   Similarly, let $|OPT(R)| = (1/b) \sum_{i = 1}^{b} |\mathcal{C}^i(R)|$ be the  optimal's length of interval inside $R$. Let $f_g$ be the total filled  time slots inside good segments and $f_b$ be total filled time slots in bad segments. 

Let $1 \le j \le b$ be the solution for which  $\sum_{i}|\mathcal{C}^j([q_i,p_{i+1}])|$ is minimum. We will replace, for each $i$,  
 $\mathcal{C}^1([q_i,p_{i+1}])$ by $\mathcal{C}^j([q_i,p_{i+1}])$ if $|\mathcal{C}^1([q_i,p_{i+1}])| > |\mathcal{C}^j([q_i,p_{i+1}])|$. We now give intution behind this. 
 Note that the original $OPT + P$ algorithm will give $OPT + P - f_b - f_g$ approximation guarantee.  This will give good approximation guarantee  if $f_b +f_g$ is large. So let us assume $f_b + f_g$ is small.  When $f_b + f_g$ is small then we know that $vol(U) =  P - f_b - f_g$ must be large. Therefore, for $R = \cup_{i = 1}^{r} [p_i,q_i]$, $|\mathcal{C}^i(R)| = f_g$ is small compared to $|OPT(R)| \ge vol(U)$.   However for any bad time segment $[q_i,p_{i+1}]$,  $|\mathcal{C}^1([q_i,p_{i+1}])|$ may be large compared to $|OPT([q_i,p_{i+1}])|$. Therefore, we do the above replacement to minimize the length of the solution.
 %Let $1 \le j \le b$ be the solution for which  $\sum_{i}|\mathcal{C}^j([q_i,p_{i+1}])|$ is minimum. We will replace, for each $i$, $\mathcal{C}^1([q_i,p_{i+1}])$ by $\mathcal{C}^j([q_i,p_{i+1}])$ if $|\mathcal{C}^1([q_i,p_{i+1}])| > \mathcal{C}^j([q_i,p_{i+1}])$.
%So what we will do is that,   we will remove $\cup_{i} \mathcal{C}^1([q_i,p_{i+1}])$ from our skelton and add $\cup_{i} \mathcal{C}^j([q_i,p_{i+1}])$ for $j$ that minimizes $\sum_{i}|\mathcal{C}^j([q_i,p_{i+1}])|$.
%This may increase the number of intervals (we may also add new intervals) but will ultimately reduce the cost. 

 %For any bad segment, number of intervals can increase by at most $1$. If the number of intervals increases (by $1$) then  
%\\ \\

Our new skelton may not be valid skelton. Some jobs that crosses $p_i$ or $q_i$ may not get covered. 
In this case, we will open an interval at $p_i$ or $q_i$ as required. The number of intervals may also increase even without opening a new interval.    % The number of intervals may increase even without opening any interval.
 For example, if there is no interval strictly inside $[q_i,p_{i+1}]$ in $\mathcal{C}^1$ but there is such interval in $\mathcal{C}^j$ then we create a new interval. It may also happen that an interval may be broken into two new intervals. For instance this may happen if an interval of $\mathcal{C}^1$ strictly contains $[q_i,p_{i+1}]$ but there is no such interval in  $\mathcal{C}^j$.
\iffalse
This can happen in following ways.
\begin{enumerate}
    \item If an interval $I$ of $\mathcal{C}^1$ strictly contains $[q_i,p_{i+1}]$ but no interval of $\mathcal{C}^j$  contains $[q_i,p_{i+1}]$. There are three possibilities: an interval of $\mathcal{C}^j$ crosses $q_i$ and start time of its next interval is after $p_{i+1}$;  an interval of $\mathcal{C}^j$ crosses $p_{i+1}$ and end time of its previous interval is before $q_{i}$; an interval of $\mathcal{C}^j$ crosses $q_i$ and next interval crosses $p_{i+1}$. 
    \item 
\end{enumerate}
\fi
%Consider a job $k$ with $r_k < p_{i+1}$ and $d_k > p_{i+1}$. 
I believe following claim to be true.
\begin{claim}
The total number of intervals in the new skelton is at most $2$ times than before. 
\end{claim}
\begin{proof}
There are $4$ ways by which the number of intervals can increase. 
\begin{enumerate}
    \item A new interval is opened at $p_i$ for some $i$. This is because there exists a job $k$ with release time $r_k$ and deadline $d_k$ such that $p_i \in [r_k,d_k]$, $r_k \in [q_{i-1},p_i]$ and $d_k \in [p_i,q_i]$. Further, no interval in $\mathcal{C}_j$ overlap job $k$ in $[q_{i-1},p_i]$ and no interval in $\mathcal{C}_1$ overlap job $k$ in $[p_i,q_i]$. In this case, there must be an interval $I_1$ in $\mathcal{C}_1$ and an interval $I_2$ in $\mathcal{C}_j$ such that $r_k \le e(I_1) \le p_i$ and $p_i \le s(I_2) \le d_k$.
    \item A new interval is opened at some $q_i$ for some $i$. This is because there exists a job $k$ with release time $r_k$ and deadline $d_k$ such that $q_i \in [r_k,d_k]$, $r_k \in [p_i,q_i]$ and $d_k \in [q_i,p_{i+1}]$. Further, no interval in $\mathcal{C}_j$ overlap job $k$ in $[q_{i},p_{i+1}]$ and no interval in $\mathcal{C}_1$ overlap job $k$ in $[p_i,q_i]$. In this case, there must be an interval $I_1$ in $\mathcal{C}_1$ and an interval $I_2$ in $\mathcal{C}_j$ such that $q_i \le s(I_1) \le d_k$ and $r_k \le e(I_2) \le q_i$.
    \item A new interval is created in $[q_i,p_{i+1}]$ as there is no interval strictly inside $[q_i,p_{i+1}]$ in $\mathcal{C}^1$ but there is such an interval $\mathcal{I}_2$ in $\mathcal{C}^j$
    \item An interval gets broken into two new intervals. This happens when an interval of $\mathcal{C}^1$  contains $[q_i,p_{i+1}]$ but there is no  interval in  $\mathcal{C}^j$ contains $[q_i,p_{i+1}]$.
\end{enumerate}
We will charge the new intervals to the existing intervals of $\mathcal{C}_1$ and show that no interval of $\mathcal{C}_1$ is charged twice.  In the first and second case, we charge the  new interval to $I_1$. In the third case, we charge it to the interval in $\mathcal{C}_1$ whose endpoint is $\le s(I_2)$ and closest to $s(I_2)$. In the fourth case, we charge on the interval that gets broken. Now we show no interval of $\mathcal{C}_1$ is charged twice.

%Suppose an interval is charged as in case 1. We will show it can not be charged then as in rest of the cases. Let the charged interval be $\mathcal{}$
 %For an interval $\mathcal{I}_1$ to be charged in both case 1 and 2, 
 Suppose an interval is charged in both case 1 and 2. This means
\end{proof}
\paragraph*{Analysis:}The new length of the skeleton is at most
$\sum_{i}|\mathcal{C}^1([p_i,q_i])| + \sum_{i} |\mathcal{C}^j([q_i,p_{i+1})| \le f_g + \sum_{i} |OPT([q_i,p_{i+1})| 
= |OPT| +f_g - \sum_{i} |OPT([p_i,q_{i}])| \le |OPT| + f_g - vol(U) = |OPT| + f_g - P +f_b + f_g = |OPT| + 2f_g + f_b - P$.

Note that our new skeleton still has $f_g$ filled jobs. So new skeleton has to be extended by $P-f_g$ to get complete schedule.  Therefore, total cost of new schedule is $|OPT|+ 2f_g + f_b - P + 2Q + P - f_g = OPT +Q + f_g +f_b$. As we seen earlier,  we also have a schedule of cost $OPT + P - f_b - f_g$.  If $f_b + f_g \ge (P - Q)/2$, the second schedule gives $OPT+P/2 +Q/2$ approximation guarantee. If $f_b + f_g < (P - Q)/2$, the first schedule also gives $OPT+P/2 +Q/2$ approximation guarantee. Thus we get $1.5$ approximation algorithm.
%If this job is not covered by our new skelton then original $\mathcal{C}^1$ must overlap job $k$ by an interval in $[q_i,p_{i+1}]$ whereas no interval of $\mathcal{C}^j$ is present in $[q_i,d_k]$. It can be checked that replacing $\mathcal{C}^1([q_i,p_{i+1}])$ by $\mathcal{C}^j([q_i,p_{i+1}])$ will not increase the number of intervals in $[q_i,p_{i+1}]$. We will open an interval at $q_i$ (if there is such job $k$). Therefore 
%no interval of $\mathcal{C}^1$ in $[p_i,q_i]$ will intersect job $k$. 
%Consider any bad segment $[q_i,p_{i+1}]$. Suppose we replace  $\mathcal{C}^1([q_i,p_{i+1}])$ by $\mathcal{C}^j([q_i,p_{i+1}])$. If the time slot $[p_{i+1},p_{i+1} + 1]$ is gap in original solution $\mathcal{C}^1$ but active in  $\mathcal{C}^j$ then the number of intervals may increase by $1$. However, in this case 



==> integralitygap.tex <==
\section{Integrality Gap Of the Linear Program}
\begin{theorem}
The integrality gap of the linear program is at least $4/3$.
\end{theorem}
\begin{proof}
Let the wake up cost be $q$. Consider $2q-1$ jobs. The release time, deadline and processing time of the jobs numbered from $1$ to $q$ are as follows. We have $r_i = 2(i-1)q+i-1$, $d_i = 2(i-1)q+i$, $p_i=1$ for all $i \in [q]$.  The release time, deadline and processing time of the jobs numbered from $q+1$ to $2q-1$ are as follows. We have $r_{q+i} = r_i =2(i-1)q+i-1$, $d_{q+i} = d_{i+1}=2iq+i+1$, $p_{q+i}=q$ for all $i \in [q-1]$.

Let $OPT$ and $OPT^*$ be the value of optimal integral and fractional solution. It is easy to see that $OPT = (q+(q-1)q) + q^2 = 2q^2$. Consider a fractional solution consisting of $q+1$ intervals ($I_1$,\dots,$I_{q+1}$) with $x_I = 1/2$ for intervals $I$. The start time and end time of first $q$ intervals are as follows. We have $s(I_i) = r_i = 2(i-1)q+i-1$ and $e(I_i) = d_i = 2(i-1)q+i$ for each $i \in [q]$. We also have $s(I_{q+1}) = 0$ and $e(I_{q+1}) = d_{q}=2(q-1)q+q$.

It is easy to see that this is a feasible fractional solution. We have $OPT^* = (q+(q-1)q)+(q+1)q/2 = 3q^2/2+q/2$. For large $q$, we have $OPT/OPT^* = 2q^2/(q^2/2) = 4/3$.
\end{proof}

We will now show that if we restrict our instance to a special case then we can also provide a matching upper bound of $4/3$. Consider the problem instances where there exists a subset of jobs $J'$ such that for each job $j \in J'$, we have $d_j - r_j = 1$ and $p_j =1$. We call such jobs as fixed jobs. Further, the time intervals $\cup_{j \in J'}[r_j,d_j]$  also need to be a skeleton. Note that the instance for our lower bound satisfy the above conditions. We now show an efficient $4/3$ approximation algorithm for these instances.

Note that any algorithm will schedule any fixed job $j \in J'$ in the time interval $[r_j,d_j]$. We call the time interval ....



